Scalable and Cost-effective Data Flow Analysis for Distributed Software: Algorithms and Applications

More and more distributed software systems are being developed and deployed today. Like other software, distributed software systems also need very strong quality assurance support. Distributed software is often very large/complex, has distributed components, and does not have a global clock. All these characteristics make it very challenging to analyze the information flow of such systems to support the software quality assurance. One challenge is that existing dynamic analysis techniques hardly scale to large distributed software systems in the real world. It is also challenging to develop cost-effective dynamic analysis approaches. There are also applicability and portability challenges for dynamic analysis algorithms/applications of distributed software. My dissertation addresses these challenges via three novel approaches to data flow analysis for distributed software. My first approach is based on measuring interprocess communications to understand distributed software behaviors and predict distributed software quality. Then, I developed a particular approach that can actually pinpoint sensitive information via multi-staged and refinement-based dynamic information flow analysis for distributed software. Finally, I explored dynamic dependence analysis for distributed systems, utilizing reinforcement learning to automatically adjust analysis configurations for scalability and better cost-effectiveness tradeoffs.

==> chapters/chapter7.tex <==
\chapter{Conclusion} \label{ch:con}
In my dissertation, I have presented three associated projects ({\distmeasure}, {\flowdist}, and {\seads}) for my overall doctoral research goal:
offering scalable and cost-effective data flow analysis to support quality assurance for common distributed software.
% providing fundamental support for quality assurance of distributed software.
To achieve this goal, I have solved the scalability, cost-effectiveness, applicability, and portability challenges first for a particular security application (i.e, information flow analysis, which is essentially a targeted data flow analysis), and then for more general problems (e.g., self-adaptation, dependence analysis) to support wider applications (e.g., software maintenance, quality assurance).
% Therefore, I has focused on three associated projects for my doctoral research: \textbf{{\distmeasure}}, \textbf{{\flowdist}}, \textbf{{\seads}}, and \textbf{{\sada}}.

First, in project \textbf{{\distmeasure}} (the expansion of \cite{fu2019measuring}), I defined interprocess communications (IPC) metrics to measure the coupling and cohesion of distributed systems and then to predict and understand their quality.
% security (and other quality factors).

Second, after understanding distributed systems through IPC metrics, I developed and evaluated a refinement-based dynamic information flow analysis framework, \textbf{{\flowdist}}~\cite{fu2021flowdist} (with two alternative designs), which could overcome applicability, portability, and scalability challenges through a multi-phase analysis strategy.

Lastly, I developed a distributed, online, continuous, and cost-effective dynamic dependence analysis framework \textbf{{\seads}}~\cite{fu2020seads} for continuously running distributed systems to achieve practical scalability and cost-effectiveness through automatically adjusting analysis configurations.
It offers self-tuning cost-effectiveness tradeoffs via a reinforcement learning method.
%, through a Q-learning (a type of reinforcement learning) strategy. 
% (with a constant reward function).
% (with a constant reward function for all executions).

% , respectively.
% that exploit pre-training results (i.e., the relative precision and analysis time costs for some configurations).
% as their training data.
% from the pre-training results (i.e., the relative precision and analysis time costs for some configurations) as the training data.




